Plug-and-Play Knowledge Injection for Pre-trained Language Models

Injecting external knowledge can improve the performance of pre-trained language models (PLMs) on various downstream NLP tasks. However, massive retraining is required to deploy new knowledge injection methods or knowledge bases for downstream tasks. In this work, we are the first to study how to improve the flexibility and efficiency of knowledge injection by reusing existing downstream models. To this end, we explore a new paradigm plug-and-play knowledge injection, where knowledge bases are injected into frozen existing downstream models by a knowledge plugin. Correspondingly, we propose a plug-and-play injection method map-tuning, which trains a mapping of knowledge embeddings to enrich model inputs with mapped embeddings while keeping model parameters frozen. Experimental results on three knowledge-driven NLP tasks show that existing injection methods are not suitable for the new paradigm, while map-tuning effectively improves the performance of downstream models. Moreover, we show that a frozen downstream model can be well adapted to different domains with different mapping networks of domain knowledge. Our code and models are available at https://github.com/THUNLP/Knowledge-Plugin.

==> content/limitation.tex <==

In this paper, we present a novel knowledge injection paradigm \emph{plug-and-play knowledge injection} for PLMs. (1) This paradigm provides an opportunity to inject knowledge into PLMs with low computational costs. Due to resource constraints, we only explore it on small PLMs, including BERT-base and RoBERTa-base. In the future, we will explore it on large-scale PLMs and aim to achieve lower computational costs.
(2) Based on this paradigm, we propose map-tuning to enhance PLMs with structured knowledge, i.e., knowledge embeddings of knowledge graphs, but we did not explore how to utilize unstructured knowledge, such as Wikipedia. In the future, we will explore designing new methods for plug-and-play injection of unstructured knowledge or even a unified method for both structured and unstructured knowledge.
(3) Following previous work on knowledge injection, we focus on information extraction tasks, including relation extraction and entity typing. Beyond these tasks, we think there are many other knowledge-intensive tasks, e.g., question answering and dialogue systems, which would also benefit from plug-and-play knowledge injection.



==> tabs/general-inject-part.tex <==

\begin{table*}[!b]
\small
\centering
\begin{tabular}{ll|llll|l|l|l}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Injection} & \multicolumn{4}{c|}{FewRel 1.0} & \multirow{2}{*}{Wiki80} & \multirow{2}{*}{Wiki-ET} & \multirow{2}{*}{EntityQuestions}\\ 
&            &     \multicolumn{1}{c}{5-1}     &      \multicolumn{1}{c}{5-5}     &     \multicolumn{1}{c}{10-1}     &     \multicolumn{1}{c|}{10-5}     &         & &   \\ 
\midrule    \multirow{3}{*}{Fine-tuning} & RA        & 91.5 ($+$0.5) & 95.5 ($+$0.4) & 85.8 ($+$0.4) & \textbf{91.7} ($+$\textbf{0.9}) & 85.9 ($-$0.2)  & 76.7 ($-$0.8)  &      \\
& K-Adapter  & 88.6 ($-$2.4) & 94.5 ($-$0.6) & 82.3 ($-$3.1) & 89.9 ($-$0.9) & 86.0 ($-$0.1) & \textbf{77.8} ($+$\textbf{0.3})  &    \\
& Map-tuning & \textbf{92.6} ($+$\textbf{1.6}) & \textbf{95.6} ($+$\textbf{0.5}) & \textbf{88.1} ($+$\textbf{2.7}) & 91.2 ($+$0.4) & \textbf{86.7} ($+$\textbf{0.6}) & 76.6 ($-$0.9)    & \\ \midrule
\multirow{3}{*}{LoRA}       & RA        & 91.3 ($+$0.6) & 95.8 ($+$0.7) & 85.0 ($+$0.1) & \textbf{92.5} ($+$\textbf{1.3}) & 83.8 ($-$1.5) & 76.8 ($-$0.7)   &   \\
& K-Adapter  & 90.0 ($-$0.7) & 94.8 ($-$0.3) & 83.4 ($-$1.5) & 89.1 ($-$2.1) & 85.0 ($-$0.3) & 77.3 ($-$0.2) & \\
& Map-tuning & \textbf{92.3} ($+$\textbf{1.6}) & \textbf{96.0} ($+$\textbf{0.9}) & \textbf{87.4} ($+$\textbf{2.5}) & 91.9 ($+$0.7) & \textbf{85.8} ($+$\textbf{0.5}) & \textbf{78.3} ($+$\textbf{0.8})  &   \\ \midrule
\multirow{3}{*}{Adapter}    & RA        & 91.7 ($+$0.5) & 95.5 ($+$0.3) & 85.8 ($-$0.4) & \textbf{92.3} ($+$\textbf{1.2})  & 85.0 ($-$0.7)  & 76.8 ($-$0.7)   &    \\
& K-Adapter  & 89.9 ($-$1.3) & 94.7 ($-$0.5) & 83.6 ($-$2.6) & 90.0 ($-$1.1) & \textbf{85.9} ($+$\textbf{0.2}) &  77.7 ($+$0.2)  &  \\
& Map-tuning & \textbf{92.6} ($+$\textbf{1.4}) & \textbf{95.8} ($+$\textbf{0.6}) & \textbf{88.2} ($+$\textbf{2.0}) & 91.8 ($+$0.7) & \textbf{85.9} ($+$\textbf{0.2}) & \textbf{79.2} ($+$\textbf{1.7})    & \\ \midrule
\multirow{3}{*}{BitFit}     & RA        & 89.5 ($+$0.3) & 95.2 ($+$0.4) & 82.7 ($-$0.3) & \textbf{91.1} ($+$\textbf{1.1}) & 81.8 ($-$0.9) & 74.0 ($-$3.1)  &  \\
& K-Adapter  & 86.4 ($-$2.8) & 93.7 ($-$1.1) & 78.8 ($-$4.2) & 87.5 ($-$2.5) & 81.5 ($-$1.2) &  77.2 ($+$0.1) & \\
& Map-tuning & \textbf{90.4} ($+$\textbf{1.2})  & \textbf{95.5} ($+$\textbf{0.7}) & \textbf{85.2} ($+$\textbf{2.2}) & 90.8 ($+$0.8) & \textbf{83.7} ($+$\textbf{1.0}) & \textbf{78.0} ($+$\textbf{0.9})  &  \\ \bottomrule
\end{tabular}
\caption{Compare Map-tuning with retrieval augmentation and K-adapter in the general plug-and-play injection.}
\label{tab:general-injection-results}
\end{table*}
